Ainur: A Framework for Repeatable End-to-End Wireless Edge Computing Testbed Research

Experimental research on wireless networking in combination with edge and cloud computing has been the subject of explosive interest in the last decade. This development has been driven by the increasing complexity of modern wireless technologies and the extensive softwarization of these through projects such as a Open Radio Access Network (O-RAN). In this context, a number of small- to mid-scale testbeds have emerged, employing a variety of technologies to target a wide array of use-cases and scenarios in the context of novel mobile communication technologies such as 5G and beyond-5G. Little work, however, has yet been devoted to developing a standard framework for wireless testbed automation which is hardware-agnostic and compatible with edge- and cloud-native technologies. Such a solution would simplify the development of new testbeds by completely or partially removing the requirement for custom management and orchestration software. In this paper, we present the first such mostly hardware-agnostic wireless testbed automation framework, Ainur. It is designed to configure, manage, orchestrate, and deploy workloads from an end-to-end perspective. Ainur is built on top of cloud-native technologies such as Docker, and is provided as FOSS to the community through the KTH-EXPECA/Ainur repository on GitHub. We demonstrate the utility of the platform with a series of scenarios, showcasing in particular its flexibility with respect to physical link definition, computation placement, and automation of arbitrarily complex experimental scenarios.

==> assumptions.tex <==
\subsection{Underlying Assumptions}\label{sec:assumptions}



In order to be able to provide as general a platform as possible for containerized workloads, and target a broad spectrum of applications and network configuration, the design of Ainur needs to make a number of assumptions about the underlying testbed platform.
In this section we will detail these assumptions, and try to provide some general context and reasoning behind each of them. 


\subsubsection{Time synchronization}
Hosts on the testbed synchronize their clocks to a central \ac{NTP} server.
This is however only required for consistent time measurements \emph{across} devices; measurements with respect to the clock of a single device (e.g.\ \ac{RTT} measurements) do not require synchronization.

\subsubsection{Network architecture}
Ainur makes strong assumptions about the layout of the testbed network.
A general overview of these can be seen in \cref{fig:network}.

In particular, the network follows a split architecture composed of two sub-networks: a control network for control plane data, and a workload data network for workload payload traffic.
It is designed like this to
\begin{enumerate*}[itemjoin={{, }}, itemjoin*={{, and }}]
    \item be able to dynamically reconfigure, segment, and route the workload data network for different experiments
    \item ensure consistent and accurate network traffic measurements (\acp{RTT}, bandwidth, etc.) on the workload data network, uncontaminated by control traffic.
\end{enumerate*}

\begin{description}[style=unboxed]
    \item[Control network]
    
    The control network, whose links are represented in orange in \cref{fig:network}, carries control plane data between the control host and the rest of the hosts on the testbed.
    It also provides internet access through a gateway router, and control plane access to the cloud instances through the control \ac{VPN} gateway (more details on this below).
    
    \item[Workload data network]
        
    This network carries data generated by the workloads deployed on the testbed, and is represented by blue links in \cref{fig:network}
    It also provides access to the workload data \ac{VPN} link to cloud instances through the workload data gateway.
    Although the physical links between devices are always present, interfaces on this network by default have no \ac{IP} addresses --- these are managed dynamically by Ainur.

    \item[Managed switch]
    
    Devices on the workload data network are interconnected through a managed switch.
    This switch is used by Ainur to change the virtual topology of the workload data network at runtime using \acp{VLAN}, for instance separating the network into front-end and back-end networks.

    In order to manage it through software, the managed switch is also connected to the control network through a single link.
    The associated interface is on a separate, exclusive \ac{VLAN}, and no data from the workload data network is allowed to enter the control network.

    \item[\ac{VPN} gateways]  
    
    Two \ac{VPN} gateways are present on the testbed; one for control traffic, and one for workload data traffic to \ac{AWS} cloud instances.
    More details on these gateways are given in \cref{sec:layer3}.
    
\end{description}

\subsubsection{Separate control host}

Ainur is executed from a host separate from hosts where the workload is actually run.
This is to avoid issues that could arise from having the control plane residing on the same physical device as the workload data plane, such as traffic cross-contamination, routing issues, etc.

\subsubsection{Workload host network capabilities}

Hosts on which workloads are to be deployed must at the very least have \emph{two} network interfaces. 
One interface is connected to the control network for remote management, and the other to the workload data network, used for workload traffic.

Workload nodes may additionally have WiFi interfaces, but that is not a requirement.

\subsubsection{Software requirements}

Hosts controlled by Ainur are assumed to have a certain set of software packages installed on them.
Most of the below assumptions can be met simply by having hosts run a modern version of Ubuntu (18.04 or later, ideally 20.04).

\begin{description}[style=unboxed]
    % \item[\ac{APT}]

    % Hosts use \ac{APT} to manage installed packages.

    \item[Netplan]
    
    Hosts use Netplan\footnote{\url{https://netplan.io/}} to manage network connections and interfaces.
    
    \item[systemd]
    
    Hosts use systemd\footnote{\url{https://www.freedesktop.org/wiki/Software/systemd/}} to manage system configurations and services.
    
    \item[Docker]
    
    Docker\footnote{\url{https://docs.docker.com/}} is installed on the hosts.
    It is configured to allow regular users to run the Docker client and the server is set up to listen on unencrypted \ac{TCP} port \num{2375} on all interfaces, in addition to the default local UNIX socket.
\end{description}

\subsubsection{Authentication}
As Ainur interacts with hosts remotely, some assumptions are made about the access to these hosts.

\begin{description}[style=unboxed]
    \item[SSH access] 
    
    The \ac{SSH} client on the control host and the \ac{SSH} servers on the controlled hosts (i.e.\ workload hosts, \ac{VPN} gateways) have been configured to allow password-less, public-key based authentication.

    \item[\texttt{sudo} access]
    
    Some of the actions executed on the remote hosts by Ainur require elevated privileges.
    The \texttt{sudo} command on the remote hosts is thus configured to allow password-less privilege escalation.

\end{description} 

\subsubsection{Fluentbit logging}

A Fluentd\footnote{\url{https://www.fluentd.org/}} or Fluentbit\footnote{\url{https://fluentbit.io/}`'} server is running on a host in the control network.
At runtime, this server receives data streams of logs from all services deployed on the workload data network and collects them into log files.

\subsubsection{Cloud integration}

Cloud integration in Ainur is done in \ac{AWS}\footnote{\url{https://aws.amazon.com/}} and the associated \texttt{boto3}\footnote{\url{https://aws.amazon.com/sdk-for-python/}} Python library.

\begin{description}[style=unboxed]
    \item[Authentication to \ac{AWS}]
    
    Credentials to \ac{AWS} exist in the execution environment of Ainur on the control hosts.
    Specifically, these are credentials that allow Ainur to fully manage:
    \begin{itemize}
        \item \ac{EC2} instances, to create and terminate required compute nodes on-the-fly;
        \item security groups, to allow remote access over \ac{SSH} and \ac{VPN} to the compute nodes;
        \item and private access keys, to securely log in to the nodes over \ac{SSH}.
    \end{itemize} 
    
    \item[\acp{AMI}]
    
    \Ac{EC2} instances deployed by Ainur are expected to be based on a Linux \ac{AMI} equipped with the similar software as the local hosts.
    Specifically:

    \begin{itemize}
        \item Docker is installed and configured for regular users and over-the-network access on \ac{TCP} port \num{2375}.
        \item Netplan and systemd are present and in use.
        \item VPNCloud\footnote{\url{https://vpncloud.ddswd.de/}} is installed (see below).
    \end{itemize}
    
    \item[\ac{VPN} gateways]
    
    In order to transparently integrate remote compute instances with the local testbed resources, Ainur uses VPNCLoud to configure tunnels to the cloud for control and workload data traffic.
    This allows the control host and hosts on the workload data network to treat cloud instances as if they resided locally on the control and workload data networks.

    \begin{description}[style=unboxed]
        \item[One gateway per network]
            
        Two gateways are present on the testbed networks, as illustrated in \cref{fig:network}; one for the control traffic \ac{VPN} link, and another for the workload data traffic \ac{VPN} link.

        \item[Public \ac{IP} address]
        
        Both gateways are reachable on the same public \ac{IP} address of the gateway router.
        The gateway router listens on two different \ac{UDP} ports and forwards data to the corresponding \ac{VPN} gateway.

        \item[Pre-shared keys]
        
        Both links share the same VPNCloud authentication parameters, in particular the pre-shared key used to initiate connections.
        
        \item[Routes] 
        
        Static routes to the control \ac{VPN} link through the corresponding gateway are configured on all devices attached to the control network.

    \end{description} 
\end{description}  

==> futurework.tex <==
\section{Future Work (ExPECA 2.0)}

\begin{description}[wide,style=nextline]
    \item[Client-Server Architecture and Microservices]
    Our current design follows a monolithic approach, in which ``layers'' of software build upon each other to reach a desired state.
    This approach is easy to understand and somewhat straightforward to implement, and works well for end-to-end experimentation.
    However, it causes a couple of problems, for example:

    \begin{enumerate}
        \item Components in the implementation are quite tightly coupled, so adding new functionality or layers in many cases implies rewritting large chunks of code.
        This also requires quite a lot of synchronization between people working on different parts of the code.
        \item It makes experimentation synchronous, and when running things over \ac{SSH}, it requires the use of tools such as \texttt{screen} or \texttt{tmux} to be able to run long experiments without having to keep the connection open at all times.
        \item We currently have no way of ensuring mutual exclusion of multiple instances of Ainur on the testbed, and implementing such functionality would probably require some sort of centralized instance tracking mechanism.
    \end{enumerate}

    I (Manuel) suggest then that for ExPECA 2.0 we switch to a distributed client-server architecture, using a microservice for each core functionality.
    In other words, we would have several smaller server applications running on potentially different hosts on the network, each handling a specific part of the functionality we need.
    For instance, we could have a ``Layer 3'' service which handles setting up \ac{IP}-layer connectivity, and another ``SDR'' service which manages the \acp{SDR}.
    Services could communicate with each other using simple HTTP \acp{API} for easy debugging, and we would have an ``Ainur'' client which orchestrates the services into an experimental run.

    This has several advantages:

    \begin{enumerate}
        \item It decouples the implementation details for each service.
        As long as the \ac{API} is well-defined, it doesn't matter how the service is implemented - we could even use different languages for different functionalities.
        \item Adding new functionality becomes simply a matter of writing a new microservice and plugging it into the existing setup.
        \item Experimentation can be done asynchronously through an ``experiment scheduler'' service which queues, runs, and then collects results from experiments.
        This service would also then ensure mutual exclusion of testbed resources.
        \item Things could be parallelized.
        Our current design is sequential, even when it doesn't need to be.
        Things that do not depend on each other could be executed in parallel (e.g. cloud and local configuration), cutting down on experiment time overhead.
        \item It would fit squarely into the design of both Docker and Kubernetes, both of which are distributed client-service architectures.
    \end{enumerate}

    \item[OpenStack/Canonical MaaS]
    
    We should really consider switching to a mature framework for bare-metal provisioning instead of doing it manually with Ansible.
    Potential options are OpenStack Ironic and Canonical Metal-as-a-Service.

    \item[Raspberry Pi SSDs]
        
    Currently our Raspberry Pis boot Ubuntu 20.04 LTS from SD cards; however this is very taxing on these storage devices, and their estimated lifetime doing this is less than a year.
    We should consider switching to the slightly more expensive option of booting the Raspberry Pis from solid-state drives.
    An alternative which I am studying would be to boot all the Raspberry Pis from a SINGLE shared storage device using iSCI and network booting (PXE). 

\end{description}

% - microservices
% - openstack
% - raspberry pi rack, shared storage?


==> outline.tex <==
\section{Proposed Paper Outline}

\begin{outline}
    \item Introduction
    \begin{outline}
        \item What is Edge computing?
        \item Introduction to Testbeds
        \item Present the ExPECA Testbed
        \item Introduce Ainur
        \begin{outline}
            \item Goals
            \item Challenges
        \end{outline}
    \end{outline}
    \item Related work
    \begin{outline}
        \item Wireless communication testbeds
        \item Cloud testbeds
        \item Other testbeds (V2X)?
        \item Associated software toolkits
    \end{outline}
    \item Ainur
    \begin{outline}
        \item Goals and Challenges
        \begin{outline}
            \item Goals
            \begin{outline}
                \item Flexible benchmarking of networking architectures.
                \item Flexible experimentation on \emph{distributed systems}.
                \item Automated deployment
                \item Automated data collection
                \item Automated scaling
                \item Automated cleanup
            \end{outline}
            \item Challenges
            \begin{outline}
                \item Obtaining 100\% clean, repeatable measurements.
                \item Defining networks from software.
                \begin{outline}
                    \item Managed switch
                    \item Fully reconfigurable network
                    \item Software-defined radios
                \end{outline}
                \item How to deploy applications -> Containers
                \item How to scale applications -> Orchestrator (Docker Swarm)
                \item How to collect data from distributed applications -> Logging and distributed storage 
            \end{outline}
        \end{outline}
        \item Overview of software architecture and general guidelines
        \begin{outline}
            \item Execution flow
            \begin{outline}
                \item Higher level overview of architecture
                \item General description of software layers
                \item Step-by-step operation of a workload deployment
            \end{outline}
            \item Underlying  assumptions
            \begin{outline}
                \item Time synchronization
                \item Split network architecture
                \item Separate management node
                \item Managed switch
                \item Management network bidirectional ping
                \item Workload network bidirectional ping
                \item Supported networks on nodes
                \begin{outline}
                    \item Ethernet
                    \item WiFi
                    \item We use ethernet to plug into the SDRs when needed
                \end{outline}
                \item Authentication
                \begin{outline}
                    \item SSH access
                    \item Passwordless sudo
                \end{outline}
                \item Software prerequisites
                \begin{outline}
                    \item Nodes need to be running a variant of Ubuntu
                    \begin{outline}
                        \item Netplan
                        \item Systemd
                    \end{outline}
                    \item Each node needs to have Docker configured
                    \begin{outline}
                        \item Listening on unencrypted TCP port 2375
                    \end{outline}
                \end{outline}
                \item Fluentbit service
                \item Cloud services
                \begin{outline}
                    \item AWS
                    \item Authentication (AWS access key)
                    \item Preconfigured EC2 instances (AMIs)
                    \item VPN tunnels to instances
                    \item Routes to tunnels
                    \item Separate VPN gateways for workload and management
                \end{outline}
                \item Internet access
            \end{outline}
            \item Software Layer Implementations
            \begin{outline}
                \item Physical Layers
                \begin{outline}
                    \item Managed switch, VLANs
                    \item SDR setups
                    \begin{outline}
                        \item WiFi
                        \item LTE
                        \item 5G
                    \end{outline}
                \end{outline}
                \item Cloud instances
                \begin{outline}
                    \item Amazon Machine Images
                    \item Docker, VPN installed.
                    \item Security groups (firewall)
                    \item Ephemeral access keys
                \end{outline}
                \item IP layer, VPN, and routing
                \begin{outline}
                    \item Assign static IP addresses
                    \item Assign static routes
                    \item Connect VPN tunnels
                \end{outline}
                \item Docker Swarm
                \begin{outline}
                    \item Select a management node
                    \item Split network traffic
                    \item Connect workload nodes
                \end{outline}
                \item Storage and logging
                \begin{outline}
                    \item Storage
                    \begin{outline}
                        \item Deploy SAMBA server
                        \item Creates a distributed Docker volume
                    \end{outline}
                    \item Logging
                \end{outline}
                \item Workload
                \begin{outline}
                    \item Parse Docker-Compose
                    \item Pull container images
                    \item Create distributed storage volumes
                    \item Deploye logging containers
                    \item Deploy and scale workload
                \end{outline}
                \item Teardown
            \end{outline}
            \item (Proposed) Workload configuration structure
            \item Workflow (how to run it?)
        \end{outline}
    \end{outline}
    \item Use cases
    \begin{outline}
        \item CLEAVE
        \item EdgeDroid
        \item Other use cases (Samie?)
    \end{outline}
    \item{Conclusion and Future Work}
    \begin{outline}
        \item ExPECA 2.0
        \begin{outline}
            \item Hardware
            \begin{outline}
                \item Server Racks
                \item Software Defined Radios
            \end{outline}
            \item Ainur 2.0?
            \begin{outline}
                \item Redesign around even more cloud-native tools?
                \item Terraform
                \item OpenStack
                \item Kubernetes
            \end{outline}
        \end{outline}
    \end{outline}
\end{outline}

==> software_layers/cloud.tex <==
\subsubsection{Cloud Instances}\label{sec:cloud}

Integration with \ac{AWS} is handled by the \mintinline{python}{CloudInstances} class.
The implementation of this class uses \verb|boto3| for interaction with the \ac{AWS}, and thus needs access to appropriate credentials\footnote{%
    \url{https://boto3.amazonaws.com/v1/documentation/api/latest/guide/credentials.html}%
}.


Each instance of this class is associated with a specific \ac{AWS} region, and manages the end-to-end lifecycle of an arbitrary number of \ac{AWS} \ac{EC2} instances on said region.
Specifically, \mintinline{python}{CloudInstances} handles
\begin{enumerate*}[itemjoin={{; }}, itemjoin*={{; and }}]
    \item configuring the necessary prerequisites for deploying the instances (security groups and private access keys)
    \item deploying the instances and waiting for them to successfully boot
    \item shutting down and terminating the instances
    \item cleaning up access keys and security groups
\end{enumerate*}.
Instances of this class can be used as context managers, automating this way the termination of instances and cleanup of resources when execution exits the \mintinline{python}{with} block.

By default, \mintinline{python}{CloudInstances} spawns instances of type \verb|t3.micro|, with at least one security group allowing inbound \ac{SSH} traffic and unrestricted traffic between instances.
The type of instances spawned can be modified at runtime, and additional security groups can be added at will.

The spawned \ac{EC2} instances are created from a preconfigured \ac{AMI}, the ID of which must be passed to the \mintinline{python}{CloudInstances} instance at runtime.
This \ac{AMI} can be either be one of the default \acp{AMI} provided by \acp{AWS} --- e.g.\ a plain Ubuntu or CentOS \ac{AMI} --- or a custom \ac{AMI} which has been preconfigured by the user.
Note that although the \mintinline{python}{CloudInstances} instance places no restrictions on the \ac{AMI} used for deploying (with the exception that it needs to be a Linux-based \ac{AMI}), components such as the VPN layer (see \cref{sec:vpn}) depending on these cloud instances might have requirements of their own.

==> software_layers/flow.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\columnwidth]{figures/flow.png}
    \caption{Execution flow of Ainur.}\label{fig:flow}
\end{figure}

\Cref{fig:flow} illustrates the execution flow of Ainur.
The software follows a mostly linear approach given its direct interaction with distinct layers of hardware and networking.
Immediately after start, Ainur reads and parses the deployment configuration and parses it into a set of various dataclasses and Python dictionaries.
Next, if deploying anything to the cloud, Ainur spawns the required number of \ac{AWS} \ac{EC2} instance.
Execution then goes on to configure the physical links, connecting hosts with each other through clever management of \acp{VLAN} and \acp{SDR}.
Once physical and/or \ac{VLAN} connections are configure, \ac{IP} addresses are assigned to devices and static routes between them are configured.
If cloud instances are used, \ac{VPN} connections are established to them.
At this stage, the testbed network is fully configured, and bidirectional traffic between any two hosts is possible over the workload data network.

The next stages deal with workload deployment, scaling, and orchestration.
A \emph{Docker Swarm}\footnote{\url{https://docs.docker.com/engine/swarm/}} is deployed on the relevant hosts on the workload data network.
On top of this Swarm, required container images are fetched from a remote repository, and distributed storage is configured across all workload hosts.
Finally, the actual containerized workload is deployed as a Docker Swarm Service Stack\footnote{\url{https://docs.docker.com/engine/swarm/stack-deploy/}}, allowing us to leverage the flexibility and utilities of this orchestration platform for automatic scaling, placement, health checking, and coordination of workloads.

In terms of actual code, in practice, most steps in \cref{fig:flow} are implemented in software as abstractions of ``layers'': each step builds upon previous steps in the flow, and provides the prerequisites steps down the line expect.
Our Python implementations of these components also frequently use the \emph{context manager}\footnote{%
    For reference, see the Python documentation on \url{https://docs.python.org/3/library/contextlib.html} and associated pages.
} pattern to ensure clean teardown of the state of the testbed and the end of the execution of Ainur.


==> software_layers/ip_layer.tex <==
\subsubsection{\ac{IP} Layer Connectivity}\label{sec:layer3}

Layer 3 connectivity, that is, \ac{IP} addressing and routing, is handled by two main components in Ainur: \mintinline{python}{LANLayer} and \mintinline{python}{VPNCloudMesh}.

\mintinline{python}{LANLayer} handles local network connectivity.
It can be used as a context manager for automatic network teardown, as well as an iterator over the hosts it manages.
This class exposes two main \ac{API} methods, \mintinline{python}{self.add_hosts()} and \mintinline{python}{self.tear_down()}:
\begin{description}[]
    \item[\mintinline{python}{LANLayer.add_hosts(self, layer2)}]
    This method takes a \mintinline{python}{PhysicalLayer} object instance and configures \ac{IP} layer connectivity on the hosts within.
    This includes assigning \ac{IP} addresses to interfaces, configuring default and static routes, as well as authenticating and connecting to the desired access point in the case of WiFi.
    The underlying implementation uses Ansible to write Netplan YAML configuration files on the target hosts and subsequently apply the network configuration.

    \item[\mintinline{python}{LANLayer.tear_down(self)}]
    Performs a clean teardown of \ac{IP} layer connectivity of the hosts managed by the instance, removing the created Netplan configuration files and reverting host network configuration to its initial state.
    When \mintinline{python}{LANLayer} is used as a context manager, this method is automatically called the moment execution leaves the \mintinline{python}{with} block.
\end{description}

\mintinline{python}{VPNCloudMesh}\label{sec:vpn} handles \ac{VPN} connectivity to running cloud instances.
It makes some strong assumptions about the presence of two preconfigured \ac{VPN} gateways on the testbed (some of these have been mentioned above, but we will repeat them here for clarity):

\begin{itemize}
    \item Two VPNCloud gateways, one for control connections and one for workload data streams, are configured and accessible on the control network.
    \item One of these gateways is additionally connected to the workload data network through a separate interface.
    \item These gateways are both listening on separate \ac{UDP} ports on a single public IP address.
    In other words, both gateways access the public internet through a single \ac{NAT} gateway, on which appropriate \ac{UDP} port forwarding rules are configured to allow \ac{VPN} traffic back into the control network.
    \item The VPNCloud connections configured on the the gateways share the same pre-shared key.
    \item The VPNCloud links belong to mutually \emph{disjoint} \acs{IP}v4 address ranges.
    % \item The gateways are assigned the first host address in the available address space of their respective \ac{VPN} links.
    % For example, if the gateway \ac{VPN} link address space is \texttt{10.0.0.0/24}, the gateway has address \texttt{10.0.0.1} on the \ac{VPN} link.
    \item Devices on the control network have been preconfigured with appropriate \ac{IP} routes to reach the control gateway and its associated \ac{VPN} link.
    \item Finally, cloud instances intended to be used with this class have VPNCloud installed on them.
\end{itemize}

After spawning cloud instances with an instance of the \mintinline{python}{CloudInstances} class described in \cref{sec:cloud}, the \mintinline{python}{VPNCloudMesh} class can be used to connect said cloud instances to the control and workload data networks of the testbed.
Instances of this class can further be used as context managers for automatic cleanup of stale links, and implement an iterator interface to access connected hosts.

The \ac{API} of this class exposes the below relevant methods:

\begin{description}[]
    \item[The \mintinline{python}{VPNCloudMesh} constructor]
    
    The constructor takes the following arguments:

    \begin{description}[font=\normalfont\ttfamily\underline]
        \item[gateway\_ip] An \texttt{IPv4Address} object corresponding to the shared public \ac{IP}v4 address of the \ac{VPN} gateways (i.e.\ the public \ac{IP} address of the \ac{NAT} gateway.)
         
        \item[vpn\_psk]
        The pre-shared key used to authenticate and encrypt traffic on the \ac{VPN} links.

        \item[ansible\_ctx~\normalfont{and} ansible\_quiet]
        Correspond to an Ansible context to use for the execution of this instances' methods (see above), and a boolean flag to suppress verbose debug output, respectively.

        \item[gw\_mgmt\_ip~\normalfont{and} gw\_wkld\_ip]
        Full \ac{IP} addresses of the \ac{VPN} links for the control and workload data networks, respectively, including subnet masks.
        These values are passed as \mintinline[breakafter=4]{python}{IPv4Interface} objects, and are used to set up correct routing tables to the cloud instances.

        \item[mgmt\_local\_net~\normalfont{and} wkld\_local\_net]
        The base addresses of the local control and workload data networks, respectively, as \mintinline[breakafter=4]{python}{IPv4Network}.
        Used to configure routing back from the cloud.

        \item[mgmt\_port~\normalfont{and} wkld\_port]
        \ac{UDP} ports on the \ac{NAT} gateway forwarded to the control and workload gateways, respectively.
    \end{description}
    
    \item[\mintinline{python}{VPNCloudMesh.connect_cloud(self, ...)}]
    
    The full signature of this method is \mintinline[breakafter=.,breakafter=_]{python}{VPNCloudMesh.connect_cloud(self, cloud_layer, host_configs)}.
    The \texttt{cloud\_layer} argument corresponds to a \mintinline{python}{CloudInstances} object instance, and the \texttt{host\_configs} to a collection of host configuration dataclasses.
    This method matches the host configurations to cloud instances in the \mintinline{python}{CloudInstances} object and connects them to to the local control and workload data networks through the two aforementioned separate \ac{VPN} links.
    The underlying implementation uses a combination of the \texttt{boto3} library and Ansible to configure appropriate security groups on the instances and subsequently initialize and connect the \ac{VPN} links.

    \item[\mintinline{python}{VPNCloudMesh.tear_down(self)}]
    This method tears down the \ac{VPN} links, disconnecting the remote instances from the gateways and removing any created routes to the cloud from local devices.
    When an instance of this class is used as a context manager, this method is automatically called at the end of the \mintinline{python}{with} block, ensuring automatic cleanup of resources.
    
\end{description}


==> software_layers/physical.tex <==
\subsubsection{Physical Layer}

This layer creates and deploy the underlying physical connections of the data network and is implemented in the \mintinline{python}{PhysicalLayer} class. 
Types of connections handled by this layer could be ethernet and WiFi links, or even an entire software-defined 4G \ac{LTE} network.

In order to ensure flexibility, we make no assumptions on the wired connections between the data hosts or radios.
On the other hand, an arbitrary data plane could require wired connections between two hosts, or a host and a radio.
Therefore, we use a managed switch at the heart of the physical layer and connect all the hosts and radios to it.
According to the data network description, the physical layer then creates the required \acp{VLAN} in the switch.

At instantiation time, this class first configures ethernet connections by creating \acp{VLAN} in the workload data network switch.
It then triggers the deployment of potential wireless connections using \mintinline{python}{WirelessConnection} objects.

A set of \mintinline{python}{WirelessConnection} instances must be provided to the constructor for deployment.
This class can be used as a context manager in a \mintinline{python}{with} statement; at the end of the block, it tears down all connections and cleans the added \acp{VLAN} from the switch.

\subsubsection{Wireless Connections}
To integrate various wireless connection schemes, we have defined the Python interface \mintinline{python}{WirelessConnection}.
It unifies the interaction of Ainur with the wireless implementation in the following aspects: 
\begin{enumerate}
    \item \textbf{\mintinline{python}{start()} and \mintinline{python}{stop()} methods:} In addition to the constructor and destructor, the implementations need to override these methods which could be called by the \mintinline{python}{PhysicalLayer}.
    The constructor is used to set the configurations by the user and these methods handle the deployment.

    \item \textbf{Data gates:} Every wireless connection implementation must identify certain network interfaces whether on radios or hosts, to act as the gate for the data plane.
    Hence, any host can exchange packets through those gates if the appropriate VLANs are created on the data network managed switch.
\end{enumerate}

Currently, WiFi and \ac{LTE} implementations are available. 
User-defined implementation for other wireless connections are possible and encouraged.

We introduce how the current implementations work in the following.

\begin{description}[style=nextline]
    \item[SDR-based WiFi Network]
    The \mintinline{python}{SDRWifi} class handles the configuration and deployment of a software-defined IEEE 802.11 network using the Mangocomm software package and its supported software-defined radios \footnote{See https://mangocomm.com/802.11-mac-phy/}.
    It lunches a Docker container on the same machine to communicate with the \acp{SDR} over the control network.
    This communication is for the configuration and monitoring the WiFi nodes.
    In a WiFi network, a radio is either \emph{station} or \emph{access point}.
    To initialize a \mintinline{python}{SDRWifi} class, the user is required to provide two lists containing the access points and station nodes instances as described below.
    
    \mintinline{python}{APSoftwareDefinedRadio} class represents a WiFi access point.
    It advertises a network with a specific SSID on a radio channel and waits for the incoming connections.

    \mintinline{python}{StationSoftwareDefinedRadio} class is used for the station WiFi nodes.
    It searches for an WiFi \ac{SSID} among the networks that are being advertised and attempts for establishing the connection.
    
    When a WiFi network is up and an station is connected, the data network interfaces of the radios behave as if an ethernet cable is connecting them.
    Thus, the client hosts and the server hosts can be on the same ip layer subnets.
    \begin{figure}[t]
        \centering
        \includegraphics[width=0.8\linewidth]{figures/wifi.png}
        \caption{An example of WiFi network topology in data network and its corresponding \acp{VLAN}}
        \label{fig:wifi}
    \end{figure}

    \item[\ac{SDR}-based \ac{LTE} Network]
    \mintinline{python}{SDRLTE} class can configure and deploy a complete software-defined \ac{LTE} network.
    The constructor must be provided with an \mintinline{python}{EPC} class, a set of \mintinline{python}{ENodeB} classes, and a set of \mintinline{python}{LTEUE} classes from the \emph{autoran} Python package\footnote{See https://github.com/samiemostafavi/autoran}.
    This package exploits the \emph{docker-py} framework to run containerized OpenAirInterface \ac{LTE} functions on remote hosts.
    Network configurations are needed in the form of Python dictionaries for the construction of \emph{autoran} classes.

    \ac{LTE} \ac{EPC} consists of HSS, MME, SPGW-U, and SPGW-C services which can be run on the same host.
    For each \ac{eNodeB} or \ac{UE}, a software-defined radio and a host for signal processing must be specified additionally.
    The resulting topology of an \ac{LTE} network in Ainur is depicted in Figure \ref{fig:lte}.
    Unlike WiFi wireless connection, due to the fact that \ac{LTE} creates an internal ip network and that introduces routing complexities, the server host and the client host cannot be on the same subnet in the ip layer.
    

    \begin{figure}[t]
        \centering
        \includegraphics[width=0.8\linewidth]{figures/lte.png}
        \caption{An example of \ac{LTE} data network topology in data network and its corresponding \acp{VLAN}}
        \label{fig:lte}
    \end{figure}




\end{description}




==> software_layers/storage_logging.tex <==
\subsubsection{Storage}\label{sec:storage}

Dynamic, distributed storage shared across testbed hosts is managed by the \mintinline{python}{ExperimentStorage} class.
This class exposes a very simple \ac{API}:
\begin{itemize}
    \item At instantiation time, the instance deploys a samba\footnote{\url{https://www.samba.org/}} server container on a specified host, using a host folder mounted inside the container for persistent storage.
    Then, on each host configured on the workload data network, it configures a Docker Volume\footnote{\url{https://docs.docker.com/storage/volumes/}} pointing to the samba server.
    These Docker Volumes are only locally available, but since they all share the same identifier, they can be included in deployment configurations and mounted on applications orchestrated with Docker Swarm (see \cref{sec:swarm} below).

    The above operations are achieved using a combination of Ansible and the \texttt{docker-py} library.

    \item The server and local volumes can all be cleanly torn down using the \mintinline{python}{tear_down()} method of the class.
    This method is also automatically called at the end of the block if this class is used in a \mintinline{python}{with} statement.
\end{itemize}


\subsubsection{Logging}\label{sec:logging}

Logging of the experiment is carried out using a containerized approach.
This is achieved through the combination of \texttt{docker-py} and \textit{FluentBit} -- an open-source and multi-platform log processor and forwarding tool.
At deployment time, Ainur configures a FluentBit client container in each workload host which captures logs produced by the workload.
These FluentBit clients are configured to listen on a \ac{TCP} port to which workload logs are forwarded by Dockers built-in FluentD logging driver\footnote{\url{https://docs.docker.com/config/containers/logging/fluentd/}}.
This means that logs are automatically captured by Docker from the \emph{standard output} of the containerized workload process.
The FluentBit client containers append metadata such as timestamp, workload name, workload host ID, to the collected logs and forward them to a central FluentBit or FluentD server.

% On the other hand, the Fluent Bit server container is configured to run persistently in the background at the logging server, unless and until a restart is necessary for some development, debug or error handling purposes. They listen to a pre-defined fluent forward port for log messages from arbitrary number of fluent clients. These logs are then segregated based on various parameters like the workload name, client name and/or log category, and are accordingly written to files in a directory structure determined by the metadata.


==> software_layers/swarm.tex <==
\subsubsection{Swarm Layer}\label{sec:swarm}

\begin{listing}[tb]
\caption{Example usage of the \mintinline{python}{DockerSwarm} class.}\label{lst:swarm:example}
\begin{minted}{python}
with DockerSwarm() as swarm:
    swarm.deploy_managers(
        hosts={
            cloudlet: {'location': 'edge'},
            aws01: {'location': 'cloud'}
        }
    )
    swarm.deploy_workers(
        hosts={
            client1: {},
            client2: {}
        },
        location='user'
    )
    swarm.pull_image('ubuntu', tag='20.04')
    swarm.deploy_workload(
        specification=workload_spec
    )
\end{minted}
\end{listing}
    

This layer handles the configuration and deployment of a Docker Swarm over the controlled hosts (including cloud instances) for the orchestration of containerized workloads.
It is implemented as a class \mintinline{python}{DockerSwarm} with appropriate methods for
\begin{enumerate*}[itemjoin={{; }}, itemjoin*={{; and }}]
    \item connecting and configuring manager and worker nodes to the Swarm
    \item fetching required Docker container images to all configured nodes
    \item finally, deploying distributed workloads as stacks of Docker containers
\end{enumerate*}.
Additionally, the class defines appropriate \mintinline{python}{__enter__} and \mintinline{python}{__exit__} magic methods allowing it to be used as a context manager.

A simple example of the usage of this class and its basic \ac{API} can be observed in \cref{lst:swarm:example}, and in the following we will detail the major steps in operating this class:
\begin{description}[]
    \item[Instantiating a \mintinline{python}{DockerSwarm} object.]
    Obtaining an instance of a Swarm object is straightforward, as the constructor takes no parameters.
    \item[Adding Swarm nodes.]
    Swarm manager and worker nodes are added through the \mintinline{python}{deploy_managers()} and \mintinline{python}{deploy_workers()} methods respectively.
    These methods take a single mandatory parameter \mintinline{python}{hosts}, corresponding a mapping from \mintinline{python}{AinurHost} instances to dictionaries of node variables in the form \mintinline[breaklines, breakafter={_}]{python}{{'label_name': 'label_value'}}.
    Additional keyword arguments are parsed as default values for labels which are assigned to all nodes.

    Note that the actual underlying Docker Swarm cluster is created on-demand at the time of the first call to \mintinline{python}{deploy_managers()}.
    This means that at least one call to \mintinline{python}{deploy_managers()} \emph{must} be made before any call to any other method of the Swarm.
    \item[Fetching required container images.]
    \mintinline{python}{DockerSwarm} provides a \mintinline{python}{pull_images()} method which takes a mandatory repository parameter, as well as an optional tag identifier, and triggers a download of the specified container image on all nodes in the Swarm.
    This method supports all repository and tag formats supported by the \verb|docker-py| library, and defaults to fetching from Docker Hub\footnote{\url{https://hub.docker.com/}} when the given repository name string does not include remote registry information.
    \item[Workload Deployment.]
    Finally the Swarm object also provides a method \mintinline[breaklines, breakafter={_}]{python}{deploy_workload()}, which takes a \emph{workload definition} and deploys the workload on the Swarm.
    Details on the workload definition and running workloads are given in \cref{sec:workload} 
\end{description}


==> software_layers/workload.tex <==
\subsubsection{Workloads}\label{sec:workload}

\begin{listing}[tb]
\caption{Workload specification example.}\label{lst:compose}
\begin{minted}{yaml}
name: FooBar
duration: '3h 15m'
version: '1.2a'
# ...
compose:
  version: '3.9'
  services:
  fooServer:
    image: 'foo:server'
    hostname: 'server.{{.Task.Slot}}'
    command: '/usr/bin/server'
    environment:
      PORT: 5000
    deploy:
      replicas: 5
      placement:
        constraints:
        - "node.labels.type==cloudlet"
    volumes:
    - type: volume
      source: FooBar
      target: /opt/foobar_data
      volume:
        nocopy: true
    # ...
\end{minted}
\end{listing}

% As previously explained, in the context of Ainur and ExPECA, we use the term \emph{workload} to refer to a collection of containerized, distributed applications deployed on the testbed for a specific amount of time.
% Ainur employ Docker Swarm for this purpose, thus leveraging  

Workloads in Ainur are defined using a dictionary of metadata containing a nested \verb|docker-compose| definition, usually provided as a YAML file.
This dictionary is parsed into a \mintinline{python}{WorkloadSpecification} dataclass, which validates the structure of the definition, and which in turn is passed to a \mintinline{python}{DockerSwarm} class instance to actually deploy the workload.

In terms of structure, the workload definition dictionary is expected to contain the following keys:

\begin{description}
    \item[name]
    A string representing an identifier for the workload, used to tag logs and stored data, as well as to identify the generated dynamic distributed storage volumes.
    All leading and trailing whitespace will be trimmed from this value at parse time.
    \item[author]
    An identifier for the author of the workload specification.
    Optional, used in logs.
    \item[email]
    Contact email for the author.
    Optional, used in logs.
    \item[url]
    URL for information related to the workload; optional.
    \item[version]
    String representing a version tag for this workload.
    Optional, but defaults to \texttt{1.0} if not specified, and is parsed into a Python \mintinline{python}{LooseVersion}object for easy manipulation in code.
    \item[max\_duration]
    Represents the maximum duration for the workload, and can be specified as any string value supported by the \texttt{pytimeparse} library\footnote{\url{https://pypi.org/project/pytimeparse/}}.
    For instance, a maximum duration of \SI{1}{\hour} and \SI{30}{\minute} could be specified as any of the following strings: \mintinline{python}{'1h 30m'}, \mintinline{python}{'1.5 h'}, \mintinline{python}{'90m'}, \mintinline{python}{'5400s'}, and so on --- see the \verb|pytimeparse| library documentation for more supported formats.
    
    This value is used as a timeout for the workload.
    The \mintinline{python}{DockerSwarm} in charge of the execution and orchestration keeps track of the time the workload has been running, forcefully tearing it down if it does not exit cleanly before it the timeout.
    This prevents workloads stuck in non-ending loops from running forever and hogging up testbed resources.

    Optional, defaults to a very liberal \mintinline{python}{'1d'} (i.e.\ \SI{24}{\hour}) if not explicitly specified.
    Note that users are strongly encouraged to explicitly define this value, as the default is subject to arbitrary change as the usage patterns of the testbed evolve.

    \item[compose]
    
    Corresponds to a nested \texttt{docker-compose v3}\footnote{\url{https://docs.docker.com/compose/compose-file/compose-file-v3/}} definition, and is the single most important component of the workload specification.
    This definition must be compliant with at least version 3 of the \texttt{docker-compose} file specification standard.
    It must additionally be fully compatible with Docker Swarm service stacks\footnote{%
        \url{https://docs.docker.com/engine/reference/commandline/stack_deploy/}%
    }, as the underlying implementation of the \mintinline{python}{DockerSwarm} class uses the \texttt{docker stack deploy} command to deploy the workload on the cluster.
    Each service in this compose specification must contain a \texttt{deploy} configuration segment detailing the scaling and placement requirements for it.
    Finally, if distributed storage has been configured using the components detailed in \cref{sec:storage}, it should be mounted on the appropriate services.
    Examples of these configurations can be seen in \cref{lst:compose}; for more details refer to the \texttt{docker-compose} online documentation.
\end{description}
